Insight into cloud processes from unsupervised classification with a rotationally invariant autoencoder

Clouds play a critical role in the Earth's energy budget and their potential changes are one of the largest uncertainties in future climate projections. However, the use of satellite observations to understand cloud feedbacks in a warming climate has been hampered by the simplicity of existing cloud classification schemes, which are based on single-pixel cloud properties rather than utilizing spatial structures and textures. Recent advances in computer vision enable the grouping of different patterns of images without using human-predefined labels, providing a novel means of automated cloud classification. This unsupervised learning approach allows discovery of unknown climate-relevant cloud patterns, and the automated processing of large datasets. We describe here the use of such methods to generate a new AI-driven Cloud Classification Atlas (AICCA), which leverages 22 years and 800 terabytes of MODIS satellite observations over the global ocean. We use a rotation-invariant cloud clustering (RICC) method to classify those observations into 42 AI-generated cloud class labels at ~100 km spatial resolution. As a case study, we use AICCA to examine a recent finding of decreasing cloudiness in a critical part of the subtropical stratocumulus deck, and show that the change is accompanied by strong trends in cloud classes.

==> Narrative/04discussion.tex <==
\section{Implications and discussion}




==> Narrative/06checklist.tex <==
\section*{Checklist}
If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \yes %~See Section~\ref{sec:results},~\ref{sec:discussion}
    %\answerTODO{\yes}
  \item Did you describe the limitations of your work?
\yes
  \item Did you discuss any potential negative societal impacts of your work? \na
    %\answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them? \yes
    %\answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results? \na
    %\answerTODO{}
 \item Did you include complete proofs of all theoretical results?
    \na
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \yes
    %\answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? \yes
    %\answerTODO{}
 \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? \no because we did not need regression tasks. 
    %\answerTODO{}
 \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \yes
    %\answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators? \yes
    %\answerTODO{}
  \item Did you mention the license of the assets? \na
    %\answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL? \na
    %\answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating? \na
    %\answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? \na
    %\answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable? \na
    %\answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable? \na
   % \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation? \na
    %\answerTODO{}
\end{enumerate}


\end{enumerate}




